Probabilistic Plan Legibility with Off-the-shelf Planners

Legible planning is the creation of plans that best disambiguate their goals from a set of other candidates from an observer's perspective. In this paper we propose a method for legible planning for arbitrary PDDL domains, by extending previous research on legibility to classical planning without requiring to construct ad-hoc planners. We also discuss how the observer perspective may be estimated through a second order theory of mind that connects the planner's and the observer's task spaces. Our solution can for example be deployed in human-robot teaming scenarios, where an autonomous robot in a team can implicitly communicate its goal by producing legible plans. We present benchmark results on several PDDL planning domains. Our results generally show that plan legibility is a trade-off with plan efficiency, however, not all planning domains allows to increase legibility in the same way and a regularizing factor to balance legibility and efficiency was proved necessary.

==> old.tex <==



\iffalse


\section{Commucation of beliefs}

\section{Method}
\label{sec:method}
As discussed in Section~\ref{sec:background}, to produce a legible plan means to find a plan $\pi$ such that its goal is easily discernible from a set of other candidates in an observer perspective; this can be expressed as:
\begin{equation}
    \pi = \mathrm{argmax}\> \mathcal{H} (\hat{y}_{\hat{g}},  P(\hat{g}_{obs}|\pi_{obs})) - \gamma |\pi_{pl}|
\end{equation}

\noindent where the first term maximizes the legibility of the plan from the observer perspective. Legibility is evaluated by 

the second term regularizes planning towards cheaper plans and is instead evaluated in the planner's perspective. $\hat{g}$ is the true goal that $\pi_{pl}$ has, that is evaluated in $\Xi_{pl}$ or from the observer perspective $\Xi_{obs}$. 

Since plan legibility is to be evaluated from the observer point of view, that in the general case uses a notation different from the one utilized by the planner, we define a second-order theory of mind $T(.)$, which allows to transform the utilized plan instance $\Xi_{pl}$ to the observer perspective of the same $\Xi_{pl}'$:
\begin{equation}
    T: \mathbf{\Xi_{pl}} (\rightarrow \mathbf{\Xi_{obs}}) \rightarrow \mathbf{\Xi_{pl}}
\end{equation}

\noindent such that
\begin{equation}
    T(\Xi_{pl}) = \Xi_{pl}'
\end{equation}
For our discussions we consider $T(.)$ to be a procedure which transforms a planning domain into its corresponding version encoded from the observer perspective. As example, $T$ could transform a particular PDDL domain by modifying its operators and predicates. 

In order to keep notations slim, we introduce a slight abuse of notation by which $T$ is used to transform also goals ($T(\hat{g}_{pl}) = \hat{g}_{obs}$) and plans ($T(\pi_{pl}) = \pi_{obs}$).

With the introduction of Eq.~\ref{eq:tom}, Eq.~\ref{eq:legibility} can be further elaborated as
\begin{equation}
    \pi = \underset{\pi_{pl} \in \Pi_{pl}}{\mathrm{argmax}}\hspace{2mm} P(T(\hat{g}_{pl})|T(\pi_{pl}))P(T(\pi_{pl})) - \gamma |\pi_{pl}|
\end{equation}


\noindent where now the plan legibility term is performed exclusively by utilizing $\Xi_{pl}$ and the theory of mind $T(.)$, i.e. locally by the planner. To implement $T$ we define two PDDL planning instances $\Xi_{pl}$ and $\Xi_{pl}'$ , such that $T(\Xi_{pl}) = \Xi_{pl}'$, that will respectively be used for planning and for evaluating the legibility of plans from the observer perspective. Plan legibility is implemented by goal recognition as described in Section~\ref{sec:plan_recogniton}. By merging Eq.~\ref{eq:goal_recognition} and Eq.~\ref{eq:legibility_tom} the resulting formulation of plan legibility thus becomes: 

\begin{equation}
    \pi = \underset{\pi_{pl} \in \Pi_{pl}}{\mathrm{argmax}}\hspace{2mm} \alpha  \frac{1}{1 + e^{-\beta R(T(\pi_{pl}), T(\hat{g}_{pl}))}} - \gamma |\pi_{pl}|
\end{equation}

Since optimization of plan legibility is performed over the plan space, solving Eq.~\ref{eq:legibility_pddl} requires to exhaustively search the plan space which can be in the general case very large. For this reason we propose a greedy procedure which iteratively builds a legible plans, by incrementally aggregating the actions that make the plan towards the true goal $\hat{g}$ most legible. This procedure is illustrated in Algorithm~\ref{alg:legible_plan}.


\fi
